Correctness Verification of Neural Networks Approximating Differential Equations

Verification of Neural Networks (NNs) that approximate the solution of Partial Differential Equations (PDEs) is a major milestone towards enhancing their trustworthiness and accelerating their deployment, especially for safety-critical systems. If successful, such NNs can become integral parts of simulation software tools which can accelerate the simulation of complex dynamic systems more than 100 times. However, the verification of these functions poses major challenges; it is not straightforward how to efficiently bound them or how to represent the derivative of the NN. This work addresses both these problems. First, we define the NN derivative as a finite difference approximation. Then, we formulate the PDE residual bounding problem alongside the Initial Value Problem's error propagation. Finally, for the first time, we tackle the problem of bounding an NN function without a priori knowledge of the output domain. For this, we build a parallel branching algorithm that combines the incomplete CROWN solver and Gradient Attack for termination and domain rejection conditions. We demonstrate the strengths and weaknesses of the proposed framework, and we suggest further work to enhance its efficiency.

==> sections/abstract.tex <==
\begin{abstract}
\JS{Revisit to fit the story and the contributions}
Verification of Neural Networks (NNs) that approximate the solution of Partial Differential Equations (PDEs) is a major milestone towards enhancing their trustworthiness. If successful, such NNs can become integral parts of simulation software tools which can accelerate the simulation of complex dynamic systems more than 100 times.  However, the verification of these functions poses many challenges: it is not straightforward how to efficiently bound them or how to represent the derivative of the NN. This work tackles both of these problems. First we define the NN derivative as a finite difference approximation. Then we formulate the PDE residual bounding problem alongside the Initial Value Problem's error propagation. Finally, we propose a novel parallel branching algorithm, that combines the incomplete CROWN solver and a Gradient Attack method with novel termination and domain rejection conditions. We demonstrate the strengths and weaknesses of the proposed framework, and we suggest further work to enhance its efficiency.
\end{abstract}

==> sections/conclusions.tex <==
\section{Conclusions}
This paper dealt with the problem of correctness verification functions that include Neural Networks function approximators, especially when partial derivatives of NNs are involved. We have shown that derivatives of Neural Networks can be represented using finite differences approximation. Then we propose an input branching algorithm, with novel stopping critira

Bounding Property \ref{prop3} for the Burger's and Schrodinger's equation, leads to the creation of large computational graphs. This, in combination with the fact that the neural networks have tanh as activation functions, makes the CROWN bounds very loose. Therefore, the branching tree, gets very large. This prevents the node rejection with Gradient Descent solutions, leading to overproduction of domains to be seen. Future work will focus on finding other heuristic-based node rejection techniques, such as proving the monotonicity of the domains etc. , so the branches' number are restricted. Moreover, bounding Neural Networks involved in finite difference approximation, may be done faster using the same bounds for the NNs that apper repetitively insight the computational graph.

==> sections/correctness_verification.tex <==
\section{Correctness Verification Of PDE approximators} \label{section_properties}

\textcolor{red}{JS: We might want to add section numbers to help the orientation.}
The following describes the formulation of the verification problem for NN-based PDE solutions. After formulating the verification problems, that is applying \eqref{corr_ver} to the PDE formulation of the previous section, we present a used approach (CROWN). Our proposed algorithm improves tractability by applying two modification, namely using finite difference approximations and input branching. Section 3.4 presents the resulting algorithm for complete correctness verification.

\subsection{Bound Propagation with CROWN}
% \textcolor{red}{We have to expain this a bit more}
Bound propagation techniques seek to give a maximum bound for the optimization problem \eqref{corr_ver}.  CROWN achieves that by back propagating the bounds from the output to the input, with respect to the intermediates' layers bounds. Furthermore, using CROWN for bound propagation is extremely effective because it is able to bound nonlinear activation functions with linear upper and lower bounds \cite{wang2021betacrown}. 

%Bound propagation is succeeded as the nonlinear activation functions into a linear upper and lower bounds \cite{wang2021betacrown}. 

The additional property that makes the method attractive is the ability to scale accurately the bound propogation well using one or more GPUs. This makes it better than a Linear Programming (LP) solver, as it can be used for a greater range of activation functions, and it scales better than an LP solver. Moreover it can be used in combination with other optimization methods, such as $\alpha$-CROWN \cite{xu2021fastalphacrown} or $\beta$-CROWN \cite{wang2021betacrown}, to make the bounds tighter.

% However, CROWN only finds an upper bound for the optimization \eqref{corr_ver}, as:
% \begin{equation}
    
% \end{equation}
By bound propagation, one is trying to find a lower bound for the optimization problem: 
\begin{equation} \label{bounds_prop}
    \min_{x \in C} f_\theta(x)
\end{equation}
where $f_\theta(x)$ expresses a NN with weights $\theta$. $C$ expresses an area around a point $\hat{x}$ as $C=\{\hat{x}: ||\hat{x}-x||_p\}$.
CROWN is a framework that has been widely used for efficient bound propagation for robustness verification of NNs. It simplifies non-linear activation functions, substituting them with a lower and upper bound. By forward and backward propagation CROWN bounds each neuron's pre-activation value. Therefore the algorithm manages to find a solution $\hat{f}$ to \eqref{bounds_prop} that is greater than the optimal solution.

Nethertheless, to find the exact solution for the optimization \eqref{bounds_prop} one needs to use a Branch-and-Bound framework. Additionally, in \eqref{corr_ver}, functions $f$, may include the partial derivatives of the NN output. Concretely, in Properties \ref{prop2}, \ref{prop3}, the derivatives cannot be expressed trivially with computational graphs. Therefore, viewing each NN, as function, we can use the widely used Finite Difference Approximation, to estimate its derivatives.

\subsection{Finite Difference Approximation with NNs}
% \textcolor{red}{Explain why we need this before we start this section}
Finite difference approximation is a numerical technique used to estimate derivatives or solve differential equations by approximating them with a discrete set of points. It involves dividing a continuous domain into a grid and replacing the derivatives in the equations with finite difference approximations derived from the function values at these grid points. By utilizing forward, backward, or central differences, depending on the specific application, this method transforms calculus problems into algebraic equations that can be solved computationally. Finite difference approximation finds extensive application in various fields like physics, engineering, finance, and computer science, providing a valuable tool for approximating solutions to differential equations that may lack analytical solutions or are too complex to solve directly. 

This finite differences method for calculating functions derivatives is widely used in the literature for solving IVPs and PDEs \cite{finitedifference}. As the task of bounding functions involves multiple partial derivatives of the parametric solution expressed by a NN, we use this method to find good approximations for the partial derivatives. This methodology, constitutes an ideal candidate for this application as it enables to forward alongside propagation of the bounds, using CROWN. Therefore, the forward derivative of a parametric function $f_\theta$ can be expressed as:
\begin{equation} \label{derivative}
    \frac{\partial f_\theta}{\partial x_i} = \lim_{h \rightarrow 0} \frac{f_\theta(x,x_i+h)-f_\theta(x, x_i)}{h}
\end{equation}
Choosing a small enough $h$, one can approximate the derivative of a given NN. However, this poses limitations. As the $h$ gets smaller, there can be overflow or underflow problems, causing round-off errors. A possible solution to this problem is to increase the number of bits representing numbers e.g. switching from 32-bit to 64-bit architecture. Still, we need to be careful, as this will also increase the memory requirements.
\subsection{Input Branching}
An essential component of the proposed framework is input branching. As the provided bounds of CROWN are perturbation-dependent \cite{zhang2018efficient}, they can be too relaxed for a large input domain. Therefore a method is needed to reduce the perturbation used in CROWN. 

The input branching methodology, that was  proposed for this, falls into the Branch and Bound (BaB) framework \cite{1960BAB}, a widely recognized method for global optimization \cite{horst1996global} and NN verification \cite{jaeckle2021neural}. These algorithms are employed to guarantee the discovery of the global minimum in the problem stated in \eqref{corr_ver}. This is achieved through iterative partitioning of the initial feasible set into smaller subsets (branching), while simultaneously calculating upper and lower bounds for the global minimum (bounding). 

Nevertheless, finding a valid stopping and node rejection condition for this application is not trivial, as we do not know the final bound a-priori. For this reason, in contrast to \cite{eiras2023provably}, we used a sample-less condition, that is based on Gradient Descent/Ascent.

% A possible alternative to our algorithm is 

\subsubsection{Gradient Attack}
Finding the worst perturbation in a region can be formulated, as an unconstrained optimization problem in \eqref{bounds_prop}, and repeated here for convenience:
\begin{equation} \label{gradient_attack}
    \min_{x} f_\theta(x)  
\end{equation}
Many methodologies have been proposed to find a possible solution to \eqref{gradient_attack}, such as Fast Gradient Sign Method (FSGM) or Projected Gradient Descent (PGSM) \cite{madry2019deep}. In this work, we considered FSGM to find possible adversarial examples, but any method in the literature can be used. 

FSGM iterates as:
\begin{equation}
    x_{t+1}=x_t+l \cdot \text{sign} ( \nabla f_{\theta} )
\end{equation}
where $x_{t}$ is the NN's input vector after $t$ iterations and $l$ is a constant called, learning step. The iteration begins from a starting point $x_0$, which usually affects the outcome. A major benefit of this methodology, is that it is massively parallelizable, for different starting points. This property can be used to increase the quality of the solution.

Using this methodology, we can acquire a local maximum of the function in Property \ref{prop3}. Therefore, we can use this methodology, as a heuristic, to discard domains that have their maximum absolute upper bound value lower than the value obtained using gradient descent.

% \ref{section_properties}. Thus, some regions that have provably lower bounds can be discarded during BaB procedures. 
% Gradient Descent/Ascent (GDA) is a technique, that is based in a first or second-order optimizer, that aims to find an input point on which NNs have the worst performance \cite{brendel2019accurate}. The Gradient Descent/Ascent is formulated as:
% \begin{equation} \label{gradient_attack}
%     \min_{x} f_\theta(x)  
% \end{equation}
% One limitation of this methodology is that, as the dimensions of the input $x$ increase, the optimization becomes increasingly difficult, as iterative first or second-order methods do not guarantee the finding of a global optima.  

% Inspired by K-means initialization techniques, a possible workaround, is to sample the space and initiate multiple parallel Gradient Descent/Ascents from different points.

% It is worth noting that, using this methodology alone, without a BaB methodology, cannot


% The drawback of iterative optimizers such as Adam, which do not guarantee the discovery of the global optimal.

\subsection{Complete Correctness Verification}
Concerning optimization expressed in \eqref{bounds_prop}, we can find its exact solution using a branch and bound algorithm. We propose a branching for the input domain of the function. Specifically, given a function $f_\theta(x)$, in each iteration the algorithm divides the input domain with bounds $[LB, UB]$ in $P$ equal pieces. Then, the algoritm runs two FSGM (one for each sign) to acquire the point with the worst performance in the area. Using CROWN, it calculates their upper and lower bounds, with respect to the bounds of the domain and discards the domains that have lower upper bound than the point given by FSGM. Each of the domains are stored in a heap, so the worst-bound domain can be acquired easily.

The algorithm continues until the first domain of the heap is a point that is found by the FSGM, or if the perturbation of this domain, has reached a predefined limit $\overline{\Theta}$. The perturbation of a domain can be defined as $\frac{(UB-LB)}{2}$. The algorithm is shown in Algorithm \ref{alg:cap}. 
% We summarize the highly parallelizable algorithm for the complete verification of PDE approximators, with general activation functions. Specifically, the stopping condition of the algorithm, is whether the algorithm explored the whole input domain in a specific resolution/perturbation size $\pi$

% One challenge for building a branching algorithm for NNs correctness verification is the limited options for stopping and node discarding criteria. However, the proposed algo
\begin{algorithm}[tb]
\caption{\textcolor{red}{Input Branching Technique}}\label{alg:cap}
\begin{algorithmic}
\Require $  f_\theta(x), LB, UB,\overline{\Theta}, P $ 

\State $\text{Get } \alpha \text{ solving \eqref{gradient_attack}}$
\State $Heap \gets (\alpha ,LB, UB)$
\State $Max \gets -\infty$
% \While{$Heap \neq \{\}$}
\While{$\frac{(UB-LB)}{2} > \overline{\Theta} \text{ or } a= Max$} 
    % \For{Processes}
        % \If{$Heap \neq \{\}$}
        % \State $\text{Get } (\alpha ,LB, UB, \Theta) \text{ from } Heap $
        \State $\text{Get } \alpha \text{ solving \eqref{gradient_attack}}$
        \State $\text{Split } [LB,UB] \text{ into } P \text{ domains}$
        \State $\text{Run CROWN on the $P$ domains} \text{ and acquire } \beta_i$
        \For{$i \in P$}
            \If{$\alpha < \beta_i$}
                \State $Heap \cup (\alpha ,LB, UB)$
            \EndIf
        \EndFor   
        \State $\text{Get } (\alpha ,LB, UB) \text{from Heap }$
    \EndWhile   
\end{algorithmic}
\end{algorithm}
In Algorithm \ref{alg:cap}, $\alpha$ denotes the bound acquired by an AA on a specific point which operates on a Region Defined by $[LB, UB]$. Moreover, $\beta_i$ are the bounds of the specific domains $A_i$, acquired by CROWN. 



==> sections/formulation.tex <==
\section{Formulation}
\JS{Ideally this describes everything that we need as prerequisites for understanding the algorithm -- that would be the PDE formulation, the structure of the NNs (PINNs?) and the target properties, we want to verify -- the less we talk about formulation things in the algorithm, the better as it is easier to understand what it is applicable to and what we want to achieve --- text needs to be improved, conciseness is good but clarity and correctness are most important. And only really relevant things should be introduced.} 

In the following section we provide the general formulation for a PDE problem. , we provide a more specific instance of this problem which is crucial in many engineering applications, namely, Initial Value Problem. , we present PINNs as a possible approximator for these problems.
% \subsection{General Form of PDEs}
% \subsection{Partial Differential Equations}
\subsection{General Partial Differential Equation Problem}

A general partial differential equation (PDE) problem involves finding a function \(\boldsymbol{u}(x, t)\) that satisfies a PDE within a given spatial domain \(\Omega\) and a time domain \((0,T)\) and is subject to the appropriate boundary and initial conditions. 

Consider the following general form of a time-dependent PDE:
\begin{equation}
    F\left(\boldsymbol{u}, \frac{\partial \boldsymbol{u}}{\partial t}, \frac{\partial \boldsymbol{u}}{\partial x}, \ldots, x, t\right) = 0, \text{for} \quad (x, t) \in \Omega \times (0, T)
\end{equation}
where \(F\) represents a differential operator combining various derivatives of \(u\) with respect to the spatial and the temporal variables.

The problem is supplemented by a general form of Robin boundary conditions, as:
\begin{equation}
    % au(0,t)+b\frac{\partial u}{\partial x}(0,t)=f(t) \quad for \quad t \in [0,T]
    B[\boldsymbol{u}](x,t)=b_0(x,t) , \text{for} \quad (x, t) \in \partial \Omega \times (0, T)
\end{equation}
and initial conditions specifying the function's behavior at \(t = 0\):
\begin{equation}
    \boldsymbol{u}(x, 0) = u_0(x), \quad \text{for} \quad x \in \Omega 
\end{equation}

\subsection{Physics Informed Neural Networks}
\textcolor{red}{JS: We should include a NN formulation as we talk about activation functions and have never defined any of it}.
PINNs are a special framework of training NNs to approximate the solution of PDEs. This framework's main ingredient is to include the boundary and initial conditions alongside the PDE residual for some points, named collocation points, in the loss function. Therefore we can denote the loss function of these NNs as:
\begin{equation}
    \mathcal{L}=\alpha \cdot \sum_{i \in N_r} F_i (\boldsymbol{u}_\theta)+ \beta \cdot \sum_{i \in N_b} B_i[\boldsymbol{u}_\theta] + \gamma \cdot \sum_{i \in N_u} (\boldsymbol{u}_\theta(x,0)-\boldsymbol{u}_0)
\end{equation}
where $\alpha,\beta,\gamma$ are constants used for the sizing of the objectives in the loss function and $N_r, N_b, N_u$ are the sets of the PDE residual, boundary, and initial condition collocation points sets, used for the model training. 
Therefore an NN $f_\theta$ with $n \in \mathbb R$ neurons and weights $\theta \in \mathbb{R}^n$, trained in this framework can be described as the approximation of the solution as
\begin{equation}
    f_\theta: (\boldsymbol{x_0}, t) \rightarrow \boldsymbol{u}_\theta
\end{equation}

\subsection{Proxy properties for PDE verification}

Correctness verification as formulated in \eqref{corr_ver}, cannot be evaluated for PDE's approximators as the ground truth solution $\boldsymbol{u}$ may not be unique, and it cannot be obtained analytically.
 
However, in \cite{eiras2023provably}, authors have formulated necessary properties of a PDE solution approximator to bound the approximation error as:

\begin{enumerate}
\item $\begin{aligned}[t]
    & \max_{x \in \Omega}|\boldsymbol{u}_{\theta}(x,0)-\boldsymbol{u}_0| \leq \delta
\end{aligned}$ \label{prop1}
\item $\begin{aligned}[t]
   & \max_{(x, t) \in \partial \Omega \times (0, T)}| B[\boldsymbol{u}_{\theta}](x,t)-b_0(x,t)| \leq \epsilon
\end{aligned}$ \label{prop2}
\item $\begin{aligned}[t]
    & \max_{(x, t) \in \Omega \times (0, T)}|F(\boldsymbol{u}_{\theta},\frac{\partial \boldsymbol{u}_{\theta}}{\partial t}, \frac{\partial \boldsymbol{u}_{\theta}}{\partial x}, \ldots,x,t)| \leq \zeta
\end{aligned}$  \label{prop3}
\end{enumerate}

As presented in \cite{eiras2023provably}, the obtained bounds on $\delta$, $\epsilon$ and $\zeta$ can empirically be related to the approximation errors. We will discuss in Section 4 the special case of IVP of ODEs, where the approximation error can be bounded using $\delta$ and $\zeta$.


==> sections/introduction.tex <==
\section{Introduction}
\JS{First try, language and content to be improved / add references / ensure that contributions are precise and convincing}
Neural networks (NN) constitute functions with great function flexibility. While this allows us to approximate a wide range of complex functions, general statements on the accuracy of the learned approximation are difficult to obtain. Correctness guarantees or correctness verification aim at providing such statements. The concept behind correctness guarantees involves determining the worst-case approximation error in the input domain and it can be formulated as an optimization problem:
\begin{equation} \label{corr_ver}
    \max_{x \in \mathcal{D}} | g(u(x)) - g(u_{\theta}(x)) |
\end{equation}
\JS{Don't we want this ultimately
\begin{equation}
    \max_{x \in \mathcal{D}} | u(x) - u_{\theta}(x) |
\end{equation}}
where $u(x)$ is the ground truth solution, $u_{\theta}(x)$ is the approximation of a NN with weights $\theta$ input domain $\mathcal{D}$. Here $x \in \mathcal{D}$ is a point in the input domain and the argument that maximizes \eqref{corr_ver} indicates where the approximator has the worst performance compared to the ground truth. To enable the application of NNs in safety critical applications like power systems, providing such guarantees will be essential. However, often, the ground truth solution itself is not available.

The solution of differential equations constitutes such a set of problems. Instead of reverting to established numerical solution schemes (cite Hairer or so), the use of NNs and PINNs has been proposed (...) for solution approximations $u_{\theta}(x)$. The verification of such solutions faces a number of limitation, namely their scalability and the reliance on differentiable activation functions in the NN. Furthermore, as $u(x)$ is generally not attainable over the entire input domain, functions or operators on the solution need to be used and these can involve derivatives of the solution.
\JS{Here, we could introduce this one then, saying that it acts as a proxy for the previous one and say that g could be basically anything but it might not be unique etc.}
\begin{equation}
    \max_{x \in \mathcal{D}} | g(u(x)) - g(u_{\theta}(x)) |
\end{equation}

In this work, we propose a verification algorithm (or just adaptations?) that can be used for verification problems involving differential operators and non-differentiable activation functions. We achieve this by utilizing a Finite Difference scheme for the approximation of involved derivatives and furthermore apply a branching technique that improves the tractability of the algorithm. We demonstrate the algorithm on two PDEs. Additionally, we test the algorithm for an ODE solution, as the obtained bounds from \eqref{corr_ver} can then be used to bound the approximation $| u(x) - u_{\theta}(x) |$.


==> sections/ivp_verification.tex <==

\section{A use case: Worst-case verification for Initial value problem of ODEs}
\JS{I think this could be a nice small section to highlight, why these verification algorithms might be useful beyond pure academic interest. -- Revisit and align with results.}
A relevant subclass of PDEs are ODEs that occur in many engineering applications, usually as initial value problems. For this subset of problems, the previously derived properties can be used to bound the approximation error of learned solutions--the desired quantity we introduced in (2).  

An Initial Value Problem (IVP) is formulated using a set of Ordinary Differential Equations (ODEs) as:
\begin{align}
    F(\boldsymbol{u}(t),\frac{d\boldsymbol{u}(t)}{dt}, t) &= \frac{d}{dt}\boldsymbol{u}(t) - f(\boldsymbol{u}(t)) \label{first_general}\\
    u(0) &= u_0 \label{second_general}
\end{align}
where $\boldsymbol{u} \in \mathbb{R}^n$ denotes the n-dimensional vector of the system's state, and the time parameter $t$ lies into an interval of interest $[0,\tau)$. We assume that function $f: \mathbb{R}^n \rightarrow \mathbb{R}^n$ is a smooth differentiable function. ODEs are a special case of the general PDE formulation since the solution does not deviate through space; they are only time-dependent functions.

%ODEs are a special case of the general PDE formulation, as the solutions are only time-dependent functions, and they do not deviate through space.

The solution $\boldsymbol{u}$ will be unique if we find the function $f$ to be globally or locally Lipschitz-continuous as:
%To ensure the uniqueness of the solution $\boldsymbol{x}$ we force function $f$ to be globally or locally Lipschitz-continuous as:
\begin{equation} \label{lipsitz}
    ||f(a)-f(b)|| \leq C ||a-b||
\end{equation}
where $C$ is the Lipschitz constant or function.

If one finds the constant or function $C$ in \eqref{lipsitz}, the motion described by $f$ will be unique for a given initial state $u_0$. That is given by the Picard-Lindelöf theorem, which ensures the existence and uniqueness of the solution inside the time interval $t \in [0,\tau)$. 

Consequently, we can denote the trajectory of the motion expressed by $f$ as:
\begin{equation} \label{solution_const}
    \boldsymbol{u}(t; \boldsymbol{u}_0)= u_0 + \int_{0}^{\tau} f(\boldsymbol{u}(t)) dt
\end{equation}
which describes the solution of the IVP given its initial state $\boldsymbol{x}_0$.
% \textcolor{red}{Nevertheless, finding the solution, as a function of initial states $\boldsymbol{x}_0$ and of time $t$. Incomplete} 

\textcolor{red}{JS: I think this deserves a few more sentences, because it actually solves a very difficult problem.}
Under these assumptions, we can then express the approximation error, [\cite{Hairer}, Ch. I, Variant of Thm. 10.2] of the IVP approximator as:
\begin{equation} \label{time_error}
    e_{rr}(t) \leq e^{Ct} \delta +\int_{0}^{\tau}e^{C(\tau-t)} \zeta(t) dt
\end{equation}

==> sections/numerical_results.tex <==

\section{Numerical Results}
For the Numerical Evaluation of the proposed framework we have trained NNs in a physics-informed manner to approximate the solution of two commonly used PDEs, namely, the Burgers equation and the Schr\"{o}dinger Equation. Additionally, we gave rigorous worst-case error guarantees for a PINN for an ODE synchronous generator model, which is widely used in Power Systems Time Domain Simulations. We empirically show that the convergence of the proposed branching algorithm, to the optimal solution of Property \ref{prop3} is faster than using the branching heuristic of $\alpha \beta$-CROWN, proposed in \cite{generalbab}, when considering NNs that have tanh or ReLU activation functions.
All the experiments took place in an Intel Xeon 24-core CPU with 72GB RAM.

\subsection{Benchmarks}
In this subsection, we briefly present the benchmarks we have used to evaluate our framework. Specifically, t

\subsubsection{Burgers Equation}
Derived from the Navier-Stokes equations for velocity fields, this one-dimensional partial differential equation (PDE) is extensively used in mathematics, fluid dynamics, nonlinear acoustics, gas dynamics, and traffic flow. It operates within a temporal domain ranging from 0 to 1 and a spatial domain spanning from -1 to 1.

Burgers' PDE problem is expressed as:
\begin{equation} \label{Burgers_res}
    \frac{\partial u(x,t)}{\partial t} + u(x,t) \frac{\partial u(x,t)} {\partial x} - \frac{0.01}{\pi} \frac{\partial^2 u(x,t)}{\partial x^2}=0
\end{equation}
\begin{equation} \label{Burgers_init_conditions}
    u(0,x)=-\sin{\pi x}
\end{equation}
\begin{equation} \label{Burgers_bound_conditions}
    u(t,-1)=u(t,1)=0
\end{equation}
\subsubsection{Schrodinger Equation}
The one-dimensional nonlinear Schrödinger equation (NLSE) is a fundamental equation in quantum mechanics and nonlinear optics, extensively studied for its rich mathematical properties and physical implications. It describes the behavior of wave packets in nonlinear media, where the wave function's evolution is influenced by both linear dispersion and nonlinear effects. Although it is 1-Dimensional it is complex-valued, meaning that the approximator must approximate both real and imaginary parts. It is formulated as:
\begin{equation} \label{Shro_res}
    i \frac{\partial u(x,t)}{\partial t} + 0.5 \frac{\partial^2 u(x,t)}{\partial x^2}+ |u(t,x)|^2 u(t,x)=0
\end{equation}
\begin{equation} \label{Shro_init_conditions}
    u(0,x)=2sech(x)
\end{equation}
\begin{equation} \label{Shro_bound_conditions_1}
    u(t,-5)=u(t,5)
\end{equation}
\begin{equation} \label{Shro_bound_conditions_2}
    \frac{\partial u(-5,t)} {\partial x}=\frac{\partial u(5,t)} {\partial x}
\end{equation}
\subsubsection{Single Machine Infinite Bus IVP}
Next we present the swing equation for the Single Machine Infinite Bus system, a system widely used in power systems to simulate and study critical dynamic phenomena. The assumption is that the generator state does not directly influence the grid-side voltage. Therefore, a voltage reference is set in the point of the connection and the active power production $P$ is able to vary without affecting the reference.. 
\begin{equation} \label{SMIB_FORMULATION}
    \left[
    \begin{matrix}
    \frac{d \delta(t)}{dt} \\
    \frac{d \Delta \omega}{dt}
    \end{matrix}
    \right] =
    \left[
    \begin{matrix}
    0 & 1 \\
    0 & -\frac{d}{m}
    \end{matrix}
    \right] 
    \left[
    \begin{matrix}
     \delta \\
    \Delta \omega
    \end{matrix}
    \right] +
    \left[
    \begin{matrix}
    0 \\
    \frac{1}{m} (P-V_1 V_2 B_{12} \sin(\delta))
    \end{matrix}
    \right]
\end{equation}
\begin{equation} \label{SMIB_init_cond}
    \delta(0) = \delta_0
\end{equation}
For this benchmark, we considered that $\Delta \omega = 0.1$ constantly. The time domain was $[0,2]$ and the $\delta_0$ take values in $[0,1]$. Moreover, network parameters were considered to be $B_{12}=0.2$ p.u., voltages $V_1=1$ p.u. and $V_2=1$ p.u., machine's damping coefficient $d=0.15$ p.u., and machine inertia constant $m=0.4$ p.u. 

As this problem is an IVP with a specific Lipschitz constant, our goal is to find how the error evolves through time, as described in \eqref{time_error}. This is important as it would possibly establish PINNs as ODE solvers, leading to the creation of novel and faster time-domain simulators such as \cite{stiasny2023pinnsim}.

\subsection{Finite Difference Approximation Quality}
To monitor the derivatives approximation quality using different values for $h$ in the equation \eqref{derivative}, we sample $10^5$ points. Then we find the averaged Minimum Square Error (MSE) of the partial derivatives, calculated by the proposed method and by autodiff differentiation of the Burgers' equation NN approximators with ReLU and Tanh activation functions. 

The results of this assessment can be seen in Figure \ref{fig:Figureders}. Specifically, from the assesment it can be seen that the difference between the two different methodologies for calculating the partial derivatives, is nearly zero, when h is taking values in $[10^{-2},10^{-7}]$. However, a major limitation of this methodology is the underflow or overflow, as the differences between the values are small enough to cause it. This can be seen for small values of $h$, where the avaraged MSE increases. Furthermore, the derivatives must be chosen small enough, to increase the quality of the derivative, as it can be shown that in \ref{subfig:lab1}-\ref{subfig:lab5} for $h=10^{-1}$ the derivative quality is low.


 \begin{figure*}[t]
        \centering
            \subfigure[] 
            {
                \label{subfig:lab1}
                \includegraphics[width=.3\textwidth]{pictures/burgurs_t_tanh.eps} % .png .jpg ... according to supported graphics files
            } 
            %
            \subfigure[] 
            {
                \label{subfig:lab2}
                \includegraphics[width=.3\textwidth]{pictures/burgurs_x_tanh.eps} % .png .jpg ... according to supported graphics files
            }
            %
            \subfigure[] 
            {
                \label{subfig:lab3}
                \includegraphics[width=.3\textwidth]{pictures/burgurs_xx_tanh.eps} % .png .jpg ... according to supported graphics files
            }\\ % for new row or line of subfigures
            %
            \subfigure[] 
            {
                \label{subfig:lab4}
                \includegraphics[width=.3\textwidth]{pictures/burgurs_t_relu.eps} % .png .jpg ... according to supported graphics files
            }
            %
            \subfigure[] 
            {
                \label{subfig:lab5}
                \includegraphics[width=.3\textwidth]{pictures/burgurs_x_relu.eps} % .png .jpg ... according to supported graphics files
            }
            %
            \subfigure[] 
            {
                \label{subfig:lab6}
                \includegraphics[width=.3\textwidth]{pictures/burgurs_xx_relu.eps} % .png .jpg ... according to supported graphics files 
            }
            %
        \caption{Averaged MSE of partial derivatives of NNs calulated by finite differences and autodiff. Figures \ref{subfig:lab1}-\ref{subfig:lab3} depict the first order partial derivatives of time and spatial variable alongside the second order spatial partial derivative, of an NN Burger's equation approximator with Tanh activation functions, respectively. Correspondingly, in \ref{subfig:lab4}-\ref{subfig:lab6} the partial derivatives of of an NN Burger's equation approximator with ReLU activation functions are shown. }
        \label{fig:Figureders}
        \end{figure*}

\subsection{Bounding Results}

In this section, we provide evidence indicating that the suggested algorithm achieves convergence to the actual solution at a faster rate compared to the leading tool, $\alpha \beta$-CROWN, with the Strong Branching (SB) and nonlinear \cite{generalbab} BaB heuristics. However, due to extended computational duration, we have established a timeout of 18000s for verifying Property \ref{prop3} and 200s for Properties \ref{prop1} and \ref{prop2}. Moreover we benchmark the proposed methodologies with a Gradient Attack from different starting points, which are taken from a grid sampling technique. Finally, we present the maximum value of the residuals, having as an input $10^{5}-10^{6}$ points, which acquired by grid sampling, the input domain.

The proposed algorithm was build to support multiprocess parallelization. Therefore, it could harness the full power of provided CPUs. For the Properties \ref{prop3}, the parallel process were 50 for each iteration. For all the derivative calculations an $h=10^-6$ was used for calculating all the first-order derivatives and the $h$ was set to $10^-3$ for all the second-order derivatives. In each process, a CROWN was splitting each domain in 4 distinct parts, which implies that $P=2$. For the $\alpha \beta- CROWN$ benchmarks, a single GPU was used, and the solver's batch size was set to 2048. All the other settings were left to their default value, except of the Burger's equation case, in which we used CROWN for all the verification process, instead of $\alpha$-CROWN.

The comparison against $\alpha \beta$-CROWN are illustrated in Table \ref{sample-table-alpha}.  The most challenging tasks involved bounding Property \ref{prop3}. This arises due to the generation of larger computational graphs, alongside the broader input domain, leading to looser bounds. It can be seen that, the proposed input branching was converging faster to the actual solution, in all three cases. However in the SMIB cases, were the proposed input branching and $\alpha \beta$-CROWN-SB were terminated, with different results. The former terminated in 281s and the latter in 79s.

In addition in Table \ref{sample-table-inco} we can view the behaviour of the proposed algorithm against FSGM and Sampling Benchmark. For the Gradient attack a value of $l=10^{-3}$ was used, and had as starting points, 100 points, spread in the whole input domain. As the test-cases' input domain is dense, we can trust that the Sampling benchmark would give a bound close the the actual bound. As detailed in the table, not every time the FSGM method is finding the worst-case error of the residuals. Consequently we choose to run it for every checked domain in Algorithm \ref{alg:cap}. Nonetheless, bounding the  Properties \ref{prop1},\ref{prop2} resulted in the algorithm terminating normally,having close results with Sampling, except of the bounding of \ref{Burgers_bound_conditions}, which ended due to the time limit.

\begin{table*}[]
\caption{Incomplete Verification Benchmarks}
\label{sample-table-inco}
\begin{center}
\begin{small}
\begin{tabular}{lcccc}
\toprule
Benchmark & Verified Conditions & Sampling & Gradient Attack & Proposed \\
\midrule
Burgers Equation & $\eqref{Burgers_init_conditions}$ & $2.312 \times 10^{-3}$ & $1.460 \times 10^{-3}$ & $2.372 \times 10^{-3}$ \\
& $\eqref{Burgers_bound_conditions}$ & $1.392 \times 10^{-2}$ & $1.636 \times 10^{-4}$ & $2.046 \times 10^{-2}$ \\
& $\eqref{Burgers_res}$ & $9.996 \times 10^{-1}$ & $6.218 \times 10^{-2}$ & $2.808 \times 10^8$ \\
\midrule
Schrodinger Equation & $\eqref{Shro_init_conditions}$ & $2.230 \times 10^{-1}$ & $2.230 \times 10^{-1}$ & $2.230 \times 10^{-1}$ \\
& $\eqref{Shro_bound_conditions_1}$ & $3.178 \times 10^{-3}$ & $3.178 \times 10^{-3}$ & $3.178 \times 10^{-3}$ \\
& $\eqref{Shro_bound_conditions_2}$ & $2.420 \times 10^{-6}$ & $2.421 \times 10^{-10}$ & $2.591 \times 10^{-6}$ \\
& $\eqref{Shro_res}$ & $2.090 \times 10^0$ & $3.891 \times 10^{-1}$ & $3.617 \times 10^3$ \\
\midrule
Single Machine Infinite Bus & $\eqref{SMIB_init_cond}$ & $5.6251 \times 10^{-1}$ & $5.6251 \times 10^{-1}$ & $5.6255 \times 10^{-1}$ \\
& $\eqref{SMIB_FORMULATION}$ & $3.086 \times 10^{-3}$ & $3.091 \times 10^{-3}$ & $3.091 \times 10^{-3}$ \\
& $e(t)$ & $8.430 \times 10^{-1}$ & $8.430 \times 10^{-1}$ & $8.430 \times 10^{-1}$ \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\end{table*}

\begin{table*}[h]
\caption{$\alpha \beta$-CROWN Benchmarks}
\label{sample-table-alpha}
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{small}
\begin{tabular}{lccccccc}
\toprule
Benchmark & Verified Conditions & Proposed (time) & $\alpha \beta$-CROWN (time)-nonlinear & $\alpha \beta$-CROWN-SB \\
\midrule
Burgers Equation &  \eqref{Burgers_res} & $2.80800 \times 10^{6}$ & $3.828 \times 10^9$ & & \\
Shroiddiger Equation & \eqref{Shro_res} & $3.617 \times 10^3$ & $1.682 \times 10^8$ & $9.497 \times 10^{4}$ & \\
Single Machine Infinite bus & \eqref{SMIB_FORMULATION} & $3.091 \times 10^{-3}$ & $7.39 \times 10^{2}$ & $9.401 \times 10^{-1} $ & \\
\bottomrule
\end{tabular}
\end{small}
}
\end{center}
\end{table*}

==> sections/related_work.tex <==
\section{Related work}
\JS{These are just copied so far, a sentence to make the point of this section clear and going through the subsection so that they fit the introduction are necessary - the question is a bit if we really need the review of the PINNs - one might argue that they work by penalising the residual but they cannot guarantee anything there ... it's like a weak verification. And of course it would be a nice training framework to combine the verification with.}

\subsection{PINNs}
A NN application domain with outstanding potential is the approximation of Partial Differential Equations (PDEs). PDEs are very useful methods for explaining complex phenomena in physics, engineering etc. Consequently, it can play a key role in the ongoing advancements of deep learning methodologies, theories, and algorithms \cite{blechschmidt2021ways}. Authors of \cite{1994NNsforPDEs} were the first to propose a NN approximator for PDE solutions. Since then, many training frameworks and NN architectures have been proposed for this task, such as ConvPDE-UQ \cite{WINOVICH2019263} and PDE-Net 2.0 \cite{LONG2019108925} .

One of the most significant training frameworks for approximating general PDEs, namely Physics Informed Neural Networks (PINNs), was proposed in \cite{RAISSI2019686}. Here, the authors included the underlying physical equations in the NN training. NNs trained in this manner have been extensively used in the literature, and they have been proven extremely effective in approximating various steady and unsteady PDEs \cite{cuomo2022scientific}. PINNs were also proven extremely useful for the approximation of Ordinary Differential Equations (ODEs) for numerous engineering applications, such as, \cite{stiasny2023physics, stiasny2023pinnsim,Nath2023} to speed up time-domain simulations by at least 10-100 times. Furthermore, in \cite{Nath2023}, a PINN was suggested to monitor diesel engine health, assess engine dynamics, and predict maintenance needs, predicting the solution of a system of ODEs.

\subsection{Verification}

\JS{Maybe a sentence to make clear what distinguishes the two -- is it local vs. global? But wouldn't that a matter of how the domain is specified?}
\subsubsection{Robustness Verification}
Robustness Verification of NNs is a field that has been widely studied in domains such as Computer Vision \cite{mu2019mnist}, Natural Language Processing \cite{Shi2020Robustness}, etc. The objective is to find changes in specific input samples that result in significant alterations to the output. This domain is classified into two categories: Complete Verification and Incomplete Verification. The result of incomplete verification is a loose lower bound to problem \eqref{corr_ver}, where $\mathcal{C}$ is considered a region around a specific input sample. On the other hand, complete verification provides the exact solution to the problem as mentioned earlier.

Bound Propagation was extensively studied in the context of incomplete verification of NN, as it gives the bounds of the output neurons of a NN, given an input domain. The incompleteness of these methods, comes from the outer-approximation of the feasible domain of the non-linear activation functions. This is done to reduce their computational burden. Interval Bound Propagation \cite{gowal2019effectiveness} and CROWN \cite{zhang2018efficient} were some of the methods that were proposed for this problem. These methods are building blocks of complete verifiers \cite{wang2021betacrown}, if they are combined with global optimization methods such as Branch and Bound \cite{1960BAB}. 

\subsubsection{Correctness Verification}
In contrast with robustness verification which aims to verify the stability of predictions within local regions around labeled points, correctness verification offers a method to verify the accuracy across the entire designated input space. It aims to validate the network's accuracy for all target inputs or identify areas where the network's predictions are inaccurate \cite{yang2019correctness}. 

PINNs correctness verification has been studied from different angles. In \cite{DeRyck2022,wang2022l2,deryck2023error}, authors have analyzed the error of PINNs as approximators for PDEs with certain properties, giving possible solutions for \eqref{corr_ver}. However, the proposed solutions suffer from scalability and tightness issues \cite{eiras2023provably}. 

On the other hand, the work carried out in \cite{eiras2023provably} is closer to the framework proposed in this paper, as it uses robustness verification tools for bounding certain properties of PINNs approximation error. However, this framework, can only be used with fully differentiable activation functions, which limits its applicability. Moreover, the paper's proposed branching algorithm, branches through the whole input domain, in contrast with this paper's proposed branching algorithm, which discards the verified domains.

